On LLM-Enhanced Mixed-Type Data Imputation with High-Order Message Passing

Missing data imputation, which aims to impute the missing values in the raw datasets to achieve the completeness of datasets, is crucial for modern data-driven models like large language models (LLMs) and has attracted increasing interest over the past decades. Despite its importance, existing solutions for missing data imputation either 1) only support numerical and categorical data or 2) show an unsatisfactory performance due to their design prioritizing text data and the lack of key properties for tabular data imputation. In this paper, we propose UnIMP, a Unified IMPutation framework that leverages LLM and high-order message passing to enhance the imputation of mixed-type data including numerical, categorical, and text data. Specifically, we first introduce a cell-oriented hypergraph to model the table. We then propose BiHMP, an efficient Bidirectional High-order Message-Passing network to aggregate global-local information and high-order relationships on the constructed hypergraph while capturing the inter-column heterogeneity and intra-column homogeneity. To effectively and efficiently align the capacity of the LLM with the information aggregated by BiHMP, we introduce Xfusion, which, together with BiHMP, acts as adapters for the LLM. We follow a pre-training and fine-tuning pipeline to train UnIMP, integrating two optimizations: chunking technique, which divides tables into smaller chunks to enhance efficiency; and progressive masking technique, which gradually adapts the model to learn more complex data patterns. Both theoretical proofs and empirical experiments on 10 real world datasets highlight the superiority of UnIMP over existing techniques.

==> 3_overview.tex <==



\section{Overview}
\label{sec:overview}



In this section, we present an overview of \netname, a unified LLM-enhanced imputation framework with high-order message-passing for mixed-type data imputation. The overall architecture of \netname~ is illustrated in Figure~\ref{fig:frameworks_overview}.
Given the incomplete raw dataset, \netname~ first utilizes the chunking technique and progressive masking to process data. Then, cell-oriented hypergraphs are constructed. 
\netname~utilize the tokenizer and LLM backbone for feature initialization and propagation, projecting both raw data and query prompts from the text space to the embedding space. 
These obtained features are processed through the BiHMP module, which iteratively runs the node-to-hyperedge layer and the hyperedge-to-node layer to aggregate both local and global information. The aggregated feature is then fused with the embedded prompts using an XFusion module. Note that BiHMP serves as an adapter for the LLM, with parameters in the LLM backbone frozen.
Finally, a projection head maps the data back to token space, and a decoding process is employed to translate the tokens into human-readable results.



==> experiment_Abalation_table.tex <==
\begin{table*}[thb] \centering
    \caption{Ablation Study}
    \vspace{-3mm}
    \label{tab:Abalation}
    \resizebox{\textwidth}{!}{
    \Huge
        \begin{tabular}{c*{4}{c}*{4}{c}*{4}{c}*{4}{c}*{4}{c}}
        \toprule
        & \multicolumn{10}{c}{\textbf{RMSE}} 
        & \multicolumn{10}{c}{\textbf{MAE}} \\
        \cmidrule(lr){2-11}\cmidrule(lr){12-21}
                               Model & \textit{Wine} & \textit{Heart} & \textit{Breast}  
                                & \textit{Car} & \textit{Wireless} & \textit{Abalone} &  \textit{Turkiye}
                               & \textit{Letter} & \textit{Chess}  & \textit{Shuttle}  
                               & \textit{Wine} & \textit{Heart} & \textit{Breast}  
                                & \textit{Car} & \textit{Wireless} & \textit{Abalone} &  \textit{Turkiye}
                               & \textit{Letter} & \textit{Chess}  & \textit{Shuttle} \\
        \midrule \midrule
    \netname~&    0.1306 & 0.3284 & 0.2079 & 0.3967 & 0.1024 & 0.0431 & 0.1777 & 0.0701 & 0.3019 & 0.0233 & 0.0925 & 0.2027 & 0.1147 & 0.3036 & 0.0665 & 0.0264 & 0.0804 & 0.0385 & 0.2275 & 0.0069 \\
w/o Calibration & 0.1326 & 0.3314 & 0.2104 & 0.4007 & 0.1044 & 0.0449 & 0.1788 & 0.0712 & 0.3120  & 0.0241 & 0.0934 & 0.2067  & 0.1158 & 0.3074 & 0.0681 & 0.0271 & 0.0832 & 0.0394 & 0.2288 & 0.0073 \\
w/o Local & 0.1643 & 0.3776 & 0.2325 & 0.4444 & 0.1447 & 0.0542 & 0.1829 & 0.1025 & 0.3389 & 0.0467 & 0.1120 & 0.2307 & 0.1366 & 0.3291 & 0.0906 & 0.0337 & 0.0872 & 0.0626 & 0.2416 & 0.0088 \\
w/o \aggname & 0.1347 & 0.3347 & 0.2159 & 0.4017 & 0.1127 & 0.0452 & 0.1803 & 0.0743 & 0.3197 & 0.0259 & 0.0962 & 0.2181 & 0.1196 & 0.3097 & 0.0702 & 0.0294 & 0.0866 & 0.0427 & 0.2298 & 0.0079 \\

        \bottomrule
    \end{tabular}
 }
 \vspace{-2mm}
\end{table*}





==> experiment_Efficiency_table.tex <==
\begin{table}\centering
    \caption{\color{blue}Imputation time evaluation (in seconds)}
    \vspace{-4mm}
    \label{tab:efficiency}
    \resizebox{0.47\textwidth}{!}{
    \Huge
        \begin{tabular}{c*{4}{c}*{4}{c}*{2}{c}}
        \toprule
        
         & \textit{Wine} & \textit{Heart} & \textit{Breast}  
                                & \textit{Car} & \textit{Wireless} & \textit{Abalone} &  \textit{Turkiye}
                               & \textit{Letter} & \textit{Chess}  & \textit{Shuttle} \\
        \midrule \midrule
TDM   & 1081  & 1144 & 1139  & 1145  & 1140  & 1141  & 1167  & 1160  & 1153  & 1176  \\
VGAIN & 234.9 & 222.8 & 224.4 & 77.26 & 223.7 & 218.5 & 212.9 & 195.2 & 205.3 & 210.0   \\
\netname  & 0.1+18.7 & 0.2+18.7 & 0.2+16.0 & 0.3+17.7    & 0.2+12.2 & 0.5+19.3 & 3.8+77.3  & 5.0+72.6 & 4.1+46.7 & 4.5+108.2\\


        \bottomrule
    \end{tabular}
    }
    \vspace{-4mm}
\end{table}

==> experiment_MCAR_table.tex <==
\begin{table*}[thb] \centering
    \caption{Results of missing data imputation (20\% MCAR)}
    \vspace{-3mm}
    \label{tab:MCAR}
    \resizebox{\textwidth}{!}{
    \Huge
        \begin{tabular}{c*{4}{c}*{4}{c}*{4}{c}*{4}{c}*{4}{c}}
        \toprule
        & \multicolumn{10}{c}{\textbf{RMSE}} 
        & \multicolumn{10}{c}{\textbf{MAE}} \\
        \cmidrule(lr){2-11}\cmidrule(lr){12-21}
                               Model & \textit{Wine} & \textit{Heart} & \textit{Breast}  
                                & \textit{Car} & \textit{Wireless} & \textit{Abalone} &  \textit{Turkiye}
                               & \textit{Letter} & \textit{Chess}  & \textit{Shuttle}  
                               & \textit{Wine} & \textit{Heart} & \textit{Breast}  
                                & \textit{Car} & \textit{Wireless} & \textit{Abalone} &  \textit{Turkiye}
                               & \textit{Letter} & \textit{Chess}  & \textit{Shuttle} \\
        \midrule \midrule
Mean   & 0.2172 & 0.5793 & 0.3208 & 0.4891 & 0.3271 & 0.1639 & 0.4393 & 0.2321 & 0.4122 & 0.0773 & 0.1563 & 0.3474 & 0.1855 & 0.3782 & 0.2361 & 0.1124 & 0.2412 & 0.1690 & 0.3144 & 0.0122 \\
KNNI   & 0.2064 & 0.5413 & 0.2983 & 0.5271 & 0.2566 & 0.1177 & 0.2313 & 0.1326 & 0.4451 & 0.0314 & 0.1483 & 0.3232 & 0.1705 & 0.5312 & 0.1839 & 0.0913 & 0.1153 & 0.0967 & 0.3217 & \textcolor{blue}{0.0052} \\
XGBI   & 0.2518 & 0.5868 & 0.3034 & 0.5322 & 0.2707 & 0.0942 & 0.2371 & 0.1403 & 0.3899 & 0.0397 & 0.1819 & 0.3522 & 0.1739 & 0.4501 & 0.1943 & 0.0782 & 0.1188 & 0.1023 & 0.3321 & 0.0057 \\
MissFI & 0.2079 & 0.5399 & 0.2912 & 0.5617 & 0.2368 & 0.1217 & 0.2282 & 0.1458 & 0.4217 & \textcolor{blue}{0.0287} & 0.1495 & 0.3223 & 0.1657 & 0.4811 & 0.1692 & 0.1003 & 0.1134 & 0.1063 & 0.3241 & \textcolor{red}{0.0041} \\
MICE   & 0.2189 & 0.4978 & 0.3092 & 0.5192 & 0.2227 & 0.1137 & 0.2374 & 0.1718 & 0.4485 & 0.0413 & 0.1576 & 0.2955 & 0.1777 & 0.4024 & 0.1587 & 0.1223 & 0.1189 & 0.1252 & 0.3932 & 0.0084 \\
MFI    & 0.2467 & 0.5654 & 0.4102 & 0.4572 & 0.3299 & 0.1327 & 0.2935 & 0.2204 & 0.3937 & 0.0651 & 0.1781 & 0.3386 & 0.2451 & 0.4183 & 0.2381 & 0.1039 & 0.1529 & 0.1605 & 0.3228 & 0.0112 \\
MIDAE  & 0.3689 & 0.5774 & 0.4564 & 0.4543 & 0.2749 & 0.0881 & 0.2219 & 0.1563 & 0.4318 & 0.0583 & 0.2685 & 0.3462 & 0.2759 & 0.3712 & 0.1974 & 0.0556 & 0.1096 & 0.1139 & 0.3327 & 0.0091 \\
VAEI   & 0.2172 & 0.4583 & 0.3316 & 0.5121 & 0.3623 & 0.0694 & 0.2176 & 0.1677 & 0.3657 & 0.0433 & 0.1563 & 0.2703 & 0.1927 & 0.3913 & 0.2621 & 0.0512 & 0.1070 & 0.1222 & 0.3121 & 0.0079 \\
HI-VAE & 0.1992 & 0.4427 & 0.2837 & 0.4361 & 0.2439 & 0.1124 & 0.1973 & 0.1606 & 0.3523 & 0.0475 & 0.1430 & 0.2603 & 0.1607 & 0.3722 & 0.1744 & 0.0807 & 0.0947 & 0.1170 & 0.2884 & 0.0104 \\
GINN   & 0.2327 & 0.5114 & 0.3117 & 0.4568 & 0.258  & 0.1821 & 0.3527 & 0.2483 & 0.3613 & 0.0512 & 0.1678 & 0.3041 & 0.1794 & 0.3548 & 0.1849 & 0.1103 & 0.1888 & 0.1808 & 0.2917 & 0.0063 \\
MIWAE  & 0.1891 & 0.4018 & 0.2514 & 0.4627 & 0.2044 & 0.0835 & –      & –      & –      & –      & 0.1356 & \textcolor{blue}{0.2342} & 0.1392 & 0.3625 & 0.1452 & 0.0542 & –      & –      & –      & –      \\
G2LGN  & 0.1724 & 0.4082 & \textcolor{blue}{0.2415} & 0.4781 & 0.1712 & 0.0622 & 0.1986 & 0.1563 & 0.3829 & 0.0467 & 0.1232 & 0.2383 & \textcolor{blue}{0.1326} & 0.3551 & 0.1206 & 0.0421 & 0.0955 & 0.0921 & 0.2738 & 0.0088 \\
GAIN   & 0.1843 & 0.4276 & 0.2625 & 0.4644 & 0.1847 & \textcolor{blue}{0.0592} & 0.1929 & \textcolor{blue}{0.1325} & 0.3589 & 0.0667 & 0.1320 & 0.2507 & 0.1466 & 0.3391 & 0.1306 & 0.0437 & 0.0920 & \textcolor{blue}{0.0966} & 0.2706 & 0.0108 \\
TDM    & 0.3144 & \textcolor{blue}{0.3909} & 0.3149 & \textcolor{blue}{0.4088} & \textcolor{blue}{0.1092} & 0.0761 & 0.2645 & 0.1476 & \textcolor{blue}{0.3113} & 0.0481 & 0.2215 & 0.2601 & 0.2177 & \textcolor{red}{0.2993} & \textcolor{blue}{0.0756} & 0.0556 & 0.1777 & 0.1101 & \textcolor{blue}{0.2337} & 0.0166 \\
VGAIN  & \textcolor{blue}{0.1678} & 0.4233 & 0.2937 & 0.4321 & 0.1773 & {0.0601} & \textcolor{blue}{0.1876} & 0.1425 & 0.3497 & {0.0305} & \textcolor{blue}{0.1198} & 0.2480 & 0.1674 & 0.3315 & 0.1251 & \textcolor{blue}{0.0372} & \textcolor{blue}{0.0888} & 0.1039 & 0.2615 & 0.0076 \\
\midrule
\netname   & \textcolor{red}{0.1306} & \textcolor{red}{0.3284} & \textcolor{red}{0.2079} & \textcolor{red}{0.3967} & \textcolor{red}{0.1024} & \textcolor{red}{0.0431} & \textcolor{red}{0.1777} & \textcolor{red}{0.0701} & \textcolor{red}{0.3019} & \textcolor{red}{0.0233} & \textcolor{red}{0.0925} & \textcolor{red}{0.2027} & \textcolor{red}{0.1147} & \textcolor{blue}{0.3036} & \textcolor{red}{0.0665} & \textcolor{red}{0.0264} & \textcolor{red}{0.0804} & \textcolor{red}{0.0385} & \textcolor{red}{0.2275} & \textcolor{black}{0.0069}\\

        \bottomrule
    \end{tabular}
 }
    \vspace{0.01em}
    \begin{flushleft}
        \footnotesize $*$ \textcolor{red}{Red} text indicates the best and \textcolor{blue}{blue} text indicates the second best result, respectively. '-' indicates the model needs more than 4 hours to obtain the result. 
    \end{flushleft}
\end{table*}





==> experiment_large_datasets.tex <==
\begin{table}\centering
    \caption{\color{blue}Performance over large datasets}
    \vspace{-4mm}
    \label{tab:large_results}
    \resizebox{0.47\textwidth}{!}{
    \Huge
        \begin{tabular}{c||ccc||cccc}
        \toprule
        
           & \multicolumn{3}{c||}{\textit{Retail}}  & \multicolumn{3}{c}{\textit{WISDM}}         \\
           \midrule 
           & {Time} & {RMSE} & {MAE} & {Time} & {RMSE} & {MAE} \\
           \midrule 
        
TDM  & 1190.8{s}   & 0.205 $\pm$ 0.019  & 0.126  $\pm$ 0.011 & 12072.6{s}  & 0.192 $\pm$ 0.018 & 0.116 $\pm$ 0.010 \\
VGAIN  & 408.2{s}  & 0.220 $\pm$ 0.027 & 0.130 $\pm$ 0.017 & 7802.1{s}   & 0.214 $\pm$ 0.028 & 0.124 $\pm$ 0.015  \\
NOMI   & 105.8s+205.2{s}  & 0.192 $\pm$ 0.019 & 0.121 $\pm$ 0.012 & 1166.3s+1456.2{s} & 0.187 $\pm$ 0.020 & 0.117  $\pm$ 0.012 \\
EDIT(NOMI) & 214.3{s} & 0.201 $\pm$ 0.022 & 0.129 $\pm$ 0.015 &  2293.5{s}  & 0.191 $\pm$ 0.021 & 0.119 $\pm$  0.013  \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-4mm}
\end{table}
